Generic non-convergence of low-temperature Ising Glauber dynamics on $\mathbb Z^2$

We study how typical convergence is, in the topological sense of Baire category, for the heat-bath Glauber dynamics of the nearest-neighbour, zero-field Ising model on $\mathbb Z^2$ started from translation-invariant initial laws. At sufficiently low positive temperature, we show that the initial laws whose evolution has both the plus and the minus phase as weak subsequential limits form a dense $G_\delta$ subset of the space of translation-invariant laws with the weak topology. Consequently, the initial laws for which the dynamics converges in distribution form a meagre set, which gives a partial answer to an open problem posed by Liggett. In particular, a large initial magnetisation does not force convergence to the plus phase, even for spatially ergodic initial laws. The proof combines equilibrium and mixing estimates of Gheissari and Sly with a periodic grid of plus spins of vanishing density and Baire's theorem, and it applies to all reversible monotone Glauber dynamics for the Ising model.

==> figures/data/sandwich_left.tex <==
% generated by make_figure_data.py -- do not edit
\fill (0,0) rectangle (3,1);
\fill (5,0) rectangle (19,1);
\fill (21,0) rectangle (35,1);
\fill (36,0) rectangle (40,1);
\fill (0,1) rectangle (3,2);
\fill (5,1) rectangle (19,2);
\fill (21,1) rectangle (35,2);
\fill (37,1) rectangle (40,2);
\fill (0,2) rectangle (3,3);
\fill (5,2) rectangle (19,3);
\fill (21,2) rectangle (35,3);
\fill (36,2) rectangle (40,3);
\fill (0,3) rectangle (3,4);
\fill (5,3) rectangle (19,4);
\fill (20,3) rectangle (35,4);
\fill (37,3) rectangle (40,4);
\fill (0,4) rectangle (3,5);
\fill (5,4) rectangle (19,5);
\fill (21,4) rectangle (35,5);
\fill (37,4) rectangle (40,5);
\fill (0,5) rectangle (3,6);
\fill (5,5) rectangle (19,6);
\fill (21,5) rectangle (35,6);
\fill (37,5) rectangle (40,6);
\fill (0,6) rectangle (3,7);
\fill (5,6) rectangle (19,7);
\fill (21,6) rectangle (35,7);
\fill (37,6) rectangle (40,7);
\fill (3,7) rectangle (4,8);
\fill (13,7) rectangle (14,8);
\fill (0,9) rectangle (3,10);
\fill (5,9) rectangle (19,10);
\fill (21,9) rectangle (35,10);
\fill (37,9) rectangle (40,10);
\fill (0,10) rectangle (3,11);
\fill (5,10) rectangle (19,11);
\fill (21,10) rectangle (35,11);
\fill (37,10) rectangle (40,11);
\fill (0,11) rectangle (3,12);
\fill (5,11) rectangle (19,12);
\fill (21,11) rectangle (35,12);
\fill (37,11) rectangle (40,12);
\fill (0,12) rectangle (3,13);
\fill (5,12) rectangle (19,13);
\fill (21,12) rectangle (35,13);
\fill (37,12) rectangle (40,13);
\fill (0,13) rectangle (3,14);
\fill (5,13) rectangle (19,14);
\fill (21,13) rectangle (35,14);
\fill (37,13) rectangle (40,14);
\fill (0,14) rectangle (4,15);
\fill (5,14) rectangle (19,15);
\fill (21,14) rectangle (35,15);
\fill (37,14) rectangle (40,15);
\fill (0,15) rectangle (3,16);
\fill (5,15) rectangle (19,16);
\fill (21,15) rectangle (35,16);
\fill (37,15) rectangle (40,16);
\fill (0,16) rectangle (3,17);
\fill (5,16) rectangle (19,17);
\fill (21,16) rectangle (35,17);
\fill (37,16) rectangle (40,17);
\fill (0,17) rectangle (3,18);
\fill (5,17) rectangle (19,18);
\fill (20,17) rectangle (36,18);
\fill (37,17) rectangle (40,18);
\fill (0,18) rectangle (3,19);
\fill (5,18) rectangle (19,19);
\fill (21,18) rectangle (35,19);
\fill (37,18) rectangle (40,19);
\fill (0,19) rectangle (3,20);
\fill (4,19) rectangle (19,20);
\fill (21,19) rectangle (35,20);
\fill (37,19) rectangle (40,20);
\fill (0,20) rectangle (3,21);
\fill (5,20) rectangle (19,21);
\fill (21,20) rectangle (35,21);
\fill (36,20) rectangle (40,21);
\fill (0,21) rectangle (3,22);
\fill (5,21) rectangle (19,22);
\fill (21,21) rectangle (35,22);
\fill (37,21) rectangle (40,22);
\fill (0,22) rectangle (3,23);
\fill (5,22) rectangle (19,23);
\fill (21,22) rectangle (35,23);
\fill (37,22) rectangle (40,23);
\fill (5,24) rectangle (6,25);
\fill (16,24) rectangle (17,25);
\fill (20,24) rectangle (22,25);
\fill (27,24) rectangle (28,25);
\fill (0,25) rectangle (3,26);
\fill (5,25) rectangle (35,26);
\fill (37,25) rectangle (40,26);
\fill (0,26) rectangle (3,27);
\fill (5,26) rectangle (19,27);
\fill (21,26) rectangle (35,27);
\fill (37,26) rectangle (40,27);
\fill (0,27) rectangle (3,28);
\fill (5,27) rectangle (19,28);
\fill (21,27) rectangle (35,28);
\fill (37,27) rectangle (40,28);
\fill (0,28) rectangle (3,29);
\fill (5,28) rectangle (19,29);
\fill (21,28) rectangle (35,29);
\fill (37,28) rectangle (40,29);
\fill (0,29) rectangle (3,30);
\fill (5,29) rectangle (19,30);
\fill (21,29) rectangle (35,30);
\fill (37,29) rectangle (40,30);
\fill (0,30) rectangle (3,31);
\fill (5,30) rectangle (19,31);
\fill (21,30) rectangle (35,31);
\fill (37,30) rectangle (40,31);
\fill (0,31) rectangle (3,32);
\fill (5,31) rectangle (19,32);
\fill (21,31) rectangle (35,32);
\fill (37,31) rectangle (40,32);
\fill (0,32) rectangle (3,33);
\fill (5,32) rectangle (19,33);
\fill (21,32) rectangle (36,33);
\fill (37,32) rectangle (40,33);
\fill (0,33) rectangle (3,34);
\fill (5,33) rectangle (19,34);
\fill (21,33) rectangle (35,34);
\fill (37,33) rectangle (40,34);
\fill (0,34) rectangle (3,35);
\fill (5,34) rectangle (19,35);
\fill (21,34) rectangle (35,35);
\fill (37,34) rectangle (40,35);
\fill (0,35) rectangle (3,36);
\fill (5,35) rectangle (19,36);
\fill (21,35) rectangle (35,36);
\fill (37,35) rectangle (40,36);
\fill (0,36) rectangle (3,37);
\fill (5,36) rectangle (19,37);
\fill (21,36) rectangle (35,37);
\fill (37,36) rectangle (40,37);
\fill (0,37) rectangle (3,38);
\fill (5,37) rectangle (19,38);
\fill (21,37) rectangle (35,38);
\fill (37,37) rectangle (40,38);
\fill (0,38) rectangle (3,39);
\fill (5,38) rectangle (19,39);
\fill (20,38) rectangle (35,39);
\fill (37,38) rectangle (40,39);
\fill (4,39) rectangle (5,40);
\fill (6,39) rectangle (8,40);


==> figures/data/sandwich_mid.tex <==
% generated by make_figure_data.py -- do not edit
\fill (1,0) rectangle (2,1);
\fill (6,0) rectangle (7,1);
\fill (8,0) rectangle (14,1);
\fill (15,0) rectangle (16,1);
\fill (18,0) rectangle (19,1);
\fill (22,0) rectangle (24,1);
\fill (25,0) rectangle (28,1);
\fill (30,0) rectangle (31,1);
\fill (32,0) rectangle (34,1);
\fill (37,0) rectangle (38,1);
\fill (0,1) rectangle (3,2);
\fill (5,1) rectangle (6,2);
\fill (9,1) rectangle (10,2);
\fill (11,1) rectangle (12,2);
\fill (14,1) rectangle (15,2);
\fill (18,1) rectangle (19,2);
\fill (22,1) rectangle (24,2);
\fill (26,1) rectangle (27,2);
\fill (29,1) rectangle (32,2);
\fill (34,1) rectangle (35,2);
\fill (37,1) rectangle (39,2);
\fill (0,2) rectangle (1,3);
\fill (5,2) rectangle (6,3);
\fill (7,2) rectangle (9,3);
\fill (14,2) rectangle (15,3);
\fill (18,2) rectangle (19,3);
\fill (23,2) rectangle (27,3);
\fill (28,2) rectangle (30,3);
\fill (32,2) rectangle (34,3);
\fill (37,2) rectangle (40,3);
\fill (7,3) rectangle (8,4);
\fill (9,3) rectangle (10,4);
\fill (13,3) rectangle (14,4);
\fill (15,3) rectangle (17,4);
\fill (18,3) rectangle (19,4);
\fill (21,3) rectangle (22,4);
\fill (24,3) rectangle (25,4);
\fill (27,3) rectangle (28,4);
\fill (29,3) rectangle (32,4);
\fill (33,3) rectangle (35,4);
\fill (37,3) rectangle (40,4);
\fill (0,4) rectangle (1,5);
\fill (6,4) rectangle (7,5);
\fill (11,4) rectangle (12,5);
\fill (14,4) rectangle (15,5);
\fill (21,4) rectangle (22,5);
\fill (23,4) rectangle (28,5);
\fill (33,4) rectangle (34,5);
\fill (37,4) rectangle (39,5);
\fill (0,5) rectangle (3,6);
\fill (7,5) rectangle (9,6);
\fill (12,5) rectangle (13,6);
\fill (15,5) rectangle (16,6);
\fill (17,5) rectangle (19,6);
\fill (23,5) rectangle (26,6);
\fill (27,5) rectangle (29,6);
\fill (30,5) rectangle (33,6);
\fill (34,5) rectangle (35,6);
\fill (38,5) rectangle (40,6);
\fill (7,6) rectangle (10,7);
\fill (11,6) rectangle (12,7);
\fill (15,6) rectangle (19,7);
\fill (22,6) rectangle (23,7);
\fill (26,6) rectangle (28,7);
\fill (30,6) rectangle (31,7);
\fill (32,6) rectangle (34,7);
\fill (0,9) rectangle (1,10);
\fill (12,9) rectangle (14,10);
\fill (15,9) rectangle (16,10);
\fill (17,9) rectangle (19,10);
\fill (23,9) rectangle (25,10);
\fill (26,9) rectangle (27,10);
\fill (28,9) rectangle (35,10);
\fill (38,9) rectangle (39,10);
\fill (0,10) rectangle (3,11);
\fill (7,10) rectangle (8,11);
\fill (15,10) rectangle (19,11);
\fill (21,10) rectangle (22,11);
\fill (24,10) rectangle (25,11);
\fill (26,10) rectangle (28,11);
\fill (30,10) rectangle (32,11);
\fill (33,10) rectangle (35,11);
\fill (37,10) rectangle (39,11);
\fill (0,11) rectangle (2,12);
\fill (6,11) rectangle (7,12);
\fill (8,11) rectangle (17,12);
\fill (18,11) rectangle (19,12);
\fill (21,11) rectangle (23,12);
\fill (24,11) rectangle (25,12);
\fill (29,11) rectangle (30,12);
\fill (32,11) rectangle (33,12);
\fill (34,11) rectangle (35,12);
\fill (37,11) rectangle (40,12);
\fill (0,12) rectangle (1,13);
\fill (2,12) rectangle (3,13);
\fill (5,12) rectangle (6,13);
\fill (8,12) rectangle (10,13);
\fill (11,12) rectangle (13,13);
\fill (14,12) rectangle (15,13);
\fill (16,12) rectangle (17,13);
\fill (18,12) rectangle (19,13);
\fill (22,12) rectangle (23,13);
\fill (24,12) rectangle (28,13);
\fill (29,12) rectangle (30,13);
\fill (38,12) rectangle (39,13);
\fill (0,13) rectangle (1,14);
\fill (2,13) rectangle (3,14);
\fill (5,13) rectangle (10,14);
\fill (11,13) rectangle (14,14);
\fill (16,13) rectangle (18,14);
\fill (27,13) rectangle (28,14);
\fill (29,13) rectangle (33,14);
\fill (37,13) rectangle (40,14);
\fill (1,14) rectangle (3,15);
\fill (5,14) rectangle (7,15);
\fill (12,14) rectangle (15,15);
\fill (25,14) rectangle (28,15);
\fill (29,14) rectangle (30,15);
\fill (31,14) rectangle (32,15);
\fill (0,15) rectangle (2,16);
\fill (5,15) rectangle (8,16);
\fill (9,15) rectangle (12,16);
\fill (13,15) rectangle (14,16);
\fill (22,15) rectangle (23,16);
\fill (24,15) rectangle (26,16);
\fill (31,15) rectangle (35,16);
\fill (38,15) rectangle (40,16);
\fill (1,16) rectangle (3,17);
\fill (5,16) rectangle (7,17);
\fill (10,16) rectangle (13,17);
\fill (15,16) rectangle (19,17);
\fill (21,16) rectangle (23,17);
\fill (25,16) rectangle (26,17);
\fill (28,16) rectangle (31,17);
\fill (37,16) rectangle (38,17);
\fill (1,17) rectangle (3,18);
\fill (7,17) rectangle (11,18);
\fill (12,17) rectangle (13,18);
\fill (14,17) rectangle (16,18);
\fill (18,17) rectangle (19,18);
\fill (22,17) rectangle (28,18);
\fill (29,17) rectangle (31,18);
\fill (32,17) rectangle (33,18);
\fill (34,17) rectangle (35,18);
\fill (38,17) rectangle (39,18);
\fill (1,18) rectangle (3,19);
\fill (6,18) rectangle (7,19);
\fill (8,18) rectangle (9,19);
\fill (11,18) rectangle (12,19);
\fill (13,18) rectangle (14,19);
\fill (17,18) rectangle (19,19);
\fill (21,18) rectangle (23,19);
\fill (24,18) rectangle (28,19);
\fill (33,18) rectangle (35,19);
\fill (37,18) rectangle (39,19);
\fill (0,19) rectangle (1,20);
\fill (5,19) rectangle (7,20);
\fill (8,19) rectangle (11,20);
\fill (13,19) rectangle (19,20);
\fill (22,19) rectangle (23,20);
\fill (25,19) rectangle (27,20);
\fill (28,19) rectangle (29,20);
\fill (31,19) rectangle (32,20);
\fill (38,19) rectangle (40,20);
\fill (1,20) rectangle (2,21);
\fill (5,20) rectangle (6,21);
\fill (7,20) rectangle (8,21);
\fill (9,20) rectangle (13,21);
\fill (14,20) rectangle (15,21);
\fill (16,20) rectangle (19,21);
\fill (22,20) rectangle (24,21);
\fill (25,20) rectangle (27,21);
\fill (31,20) rectangle (32,21);
\fill (33,20) rectangle (35,21);
\fill (37,20) rectangle (40,21);
\fill (0,21) rectangle (1,22);
\fill (5,21) rectangle (7,22);
\fill (8,21) rectangle (10,22);
\fill (13,21) rectangle (14,22);
\fill (15,21) rectangle (16,22);
\fill (17,21) rectangle (18,22);
\fill (21,21) rectangle (24,22);
\fill (26,21) rectangle (27,22);
\fill (28,21) rectangle (32,22);
\fill (37,21) rectangle (38,22);
\fill (0,22) rectangle (1,23);
\fill (6,22) rectangle (7,23);
\fill (8,22) rectangle (10,23);
\fill (12,22) rectangle (14,23);
\fill (15,22) rectangle (16,23);
\fill (17,22) rectangle (19,23);
\fill (21,22) rectangle (22,23);
\fill (24,22) rectangle (26,23);
\fill (29,22) rectangle (31,23);
\fill (33,22) rectangle (34,23);
\fill (0,25) rectangle (3,26);
\fill (5,25) rectangle (6,26);
\fill (9,25) rectangle (13,26);
\fill (17,25) rectangle (18,26);
\fill (24,25) rectangle (25,26);
\fill (28,25) rectangle (29,26);
\fill (31,25) rectangle (32,26);
\fill (34,25) rectangle (35,26);
\fill (0,26) rectangle (3,27);
\fill (5,26) rectangle (9,27);
\fill (11,26) rectangle (13,27);
\fill (17,26) rectangle (18,27);
\fill (22,26) rectangle (26,27);
\fill (27,26) rectangle (28,27);
\fill (29,26) rectangle (30,27);
\fill (31,26) rectangle (35,27);
\fill (38,26) rectangle (40,27);
\fill (2,27) rectangle (3,28);
\fill (6,27) rectangle (11,28);
\fill (13,27) rectangle (14,28);
\fill (16,27) rectangle (17,28);
\fill (18,27) rectangle (19,28);
\fill (23,27) rectangle (25,28);
\fill (26,27) rectangle (29,28);
\fill (31,27) rectangle (32,28);
\fill (33,27) rectangle (34,28);
\fill (37,27) rectangle (39,28);
\fill (0,28) rectangle (3,29);
\fill (10,28) rectangle (12,29);
\fill (13,28) rectangle (14,29);
\fill (16,28) rectangle (17,29);
\fill (18,28) rectangle (19,29);
\fill (21,28) rectangle (24,29);
\fill (29,28) rectangle (32,29);
\fill (33,28) rectangle (34,29);
\fill (39,28) rectangle (40,29);
\fill (0,29) rectangle (1,30);
\fill (6,29) rectangle (7,30);
\fill (9,29) rectangle (10,30);
\fill (11,29) rectangle (12,30);
\fill (14,29) rectangle (17,30);
\fill (21,29) rectangle (22,30);
\fill (23,29) rectangle (27,30);
\fill (28,29) rectangle (30,30);
\fill (31,29) rectangle (33,30);
\fill (39,29) rectangle (40,30);
\fill (0,30) rectangle (1,31);
\fill (5,30) rectangle (7,31);
\fill (9,30) rectangle (10,31);
\fill (11,30) rectangle (17,31);
\fill (18,30) rectangle (19,31);
\fill (21,30) rectangle (23,31);
\fill (25,30) rectangle (26,31);
\fill (27,30) rectangle (28,31);
\fill (29,30) rectangle (30,31);
\fill (33,30) rectangle (34,31);
\fill (37,30) rectangle (38,31);
\fill (0,31) rectangle (1,32);
\fill (2,31) rectangle (3,32);
\fill (5,31) rectangle (6,32);
\fill (8,31) rectangle (9,32);
\fill (11,31) rectangle (13,32);
\fill (17,31) rectangle (18,32);
\fill (22,31) rectangle (23,32);
\fill (27,31) rectangle (28,32);
\fill (30,31) rectangle (32,32);
\fill (39,31) rectangle (40,32);
\fill (2,32) rectangle (3,33);
\fill (5,32) rectangle (6,33);
\fill (8,32) rectangle (13,33);
\fill (15,32) rectangle (18,33);
\fill (22,32) rectangle (23,33);
\fill (24,32) rectangle (27,33);
\fill (0,33) rectangle (2,34);
\fill (5,33) rectangle (6,34);
\fill (7,33) rectangle (9,34);
\fill (11,33) rectangle (12,34);
\fill (14,33) rectangle (16,34);
\fill (18,33) rectangle (19,34);
\fill (21,33) rectangle (24,34);
\fill (26,33) rectangle (33,34);
\fill (39,33) rectangle (40,34);
\fill (0,34) rectangle (2,35);
\fill (5,34) rectangle (7,35);
\fill (14,34) rectangle (15,35);
\fill (16,34) rectangle (18,35);
\fill (22,34) rectangle (29,35);
\fill (30,34) rectangle (31,35);
\fill (33,34) rectangle (35,35);
\fill (0,35) rectangle (1,36);
\fill (2,35) rectangle (3,36);
\fill (6,35) rectangle (8,36);
\fill (9,35) rectangle (11,36);
\fill (12,35) rectangle (18,36);
\fill (21,35) rectangle (23,36);
\fill (26,35) rectangle (28,36);
\fill (29,35) rectangle (32,36);
\fill (33,35) rectangle (35,36);
\fill (38,35) rectangle (40,36);
\fill (0,36) rectangle (2,37);
\fill (5,36) rectangle (9,37);
\fill (10,36) rectangle (11,37);
\fill (12,36) rectangle (13,37);
\fill (15,36) rectangle (16,37);
\fill (17,36) rectangle (19,37);
\fill (22,36) rectangle (25,37);
\fill (28,36) rectangle (29,37);
\fill (32,36) rectangle (34,37);
\fill (37,36) rectangle (40,37);
\fill (0,37) rectangle (2,38);
\fill (7,37) rectangle (8,38);
\fill (9,37) rectangle (12,38);
\fill (14,37) rectangle (15,38);
\fill (16,37) rectangle (18,38);
\fill (21,37) rectangle (23,38);
\fill (25,37) rectangle (26,38);
\fill (27,37) rectangle (30,38);
\fill (31,37) rectangle (32,38);
\fill (34,37) rectangle (35,38);
\fill (37,37) rectangle (38,38);
\fill (0,38) rectangle (2,39);
\fill (6,38) rectangle (7,39);
\fill (8,38) rectangle (14,39);
\fill (15,38) rectangle (17,39);
\fill (21,38) rectangle (22,39);
\fill (25,38) rectangle (27,39);
\fill (28,38) rectangle (30,39);
\fill (33,38) rectangle (34,39);


==> figures/data/sandwich_params.tex <==
% generated by make_figure_data.py -- do not edit
\def\figSandN{40}\def\figSandL{14}\def\figSandP{16}\def\figSandAX{5}\def\figSandAY{9}


==> figures/data/square_interface.tex <==
% generated by make_figure_data.py -- do not edit
\fill[figMinusLight] plot[smooth cycle, tension=0.5] coordinates {(-2.265,-2.265) (-1.862,-2.284) (-1.523,-2.262) (-1.185,-2.285) (-0.846,-2.292) (-0.508,-2.273) (-0.169,-2.285) (0.169,-2.340) (0.508,-2.355) (0.846,-2.344) (1.185,-2.313) (1.523,-2.272) (1.862,-2.258) (2.265,-2.265) (2.255,-1.862) (2.246,-1.523) (2.355,-1.185) (2.254,-0.846) (2.306,-0.508) (2.290,-0.169) (2.249,0.169) (2.267,0.508) (2.274,0.846) (2.285,1.185) (2.268,1.523) (2.261,1.862) (2.265,2.265) (1.862,2.288) (1.523,2.253) (1.185,2.295) (0.846,2.301) (0.508,2.283) (0.169,2.327) (-0.169,2.342) (-0.508,2.344) (-0.846,2.355) (-1.185,2.335) (-1.523,2.297) (-1.862,2.275) (-2.265,2.265) (-2.321,1.862) (-2.278,1.523) (-2.314,1.185) (-2.279,0.846) (-2.330,0.508) (-2.323,0.169) (-2.355,-0.169) (-2.322,-0.508) (-2.257,-0.846) (-2.299,-1.185) (-2.253,-1.523) (-2.311,-1.862)};
\draw[figInterface, semithick] plot[smooth cycle, tension=0.5] coordinates {(-2.265,-2.265) (-1.862,-2.284) (-1.523,-2.262) (-1.185,-2.285) (-0.846,-2.292) (-0.508,-2.273) (-0.169,-2.285) (0.169,-2.340) (0.508,-2.355) (0.846,-2.344) (1.185,-2.313) (1.523,-2.272) (1.862,-2.258) (2.265,-2.265) (2.255,-1.862) (2.246,-1.523) (2.355,-1.185) (2.254,-0.846) (2.306,-0.508) (2.290,-0.169) (2.249,0.169) (2.267,0.508) (2.274,0.846) (2.285,1.185) (2.268,1.523) (2.261,1.862) (2.265,2.265) (1.862,2.288) (1.523,2.253) (1.185,2.295) (0.846,2.301) (0.508,2.283) (0.169,2.327) (-0.169,2.342) (-0.508,2.344) (-0.846,2.355) (-1.185,2.335) (-1.523,2.297) (-1.862,2.275) (-2.265,2.265) (-2.321,1.862) (-2.278,1.523) (-2.314,1.185) (-2.279,0.846) (-2.330,0.508) (-2.323,0.169) (-2.355,-0.169) (-2.322,-0.508) (-2.257,-0.846) (-2.299,-1.185) (-2.253,-1.523) (-2.311,-1.862)};
\def\figSquareExcX{-0.846}
\def\figSquareExcY{2.355}

